Framing image registration as a landmark detection problem for label-noise-aware task representation (HitR)

Accurate image registration is pivotal in biomedical image analysis, where selecting suitable registration algorithms demands careful consideration. While numerous algorithms are available, the evaluation metrics to assess their performance have remained relatively static. This study addresses this challenge by introducing a novel evaluation metric termed Landmark Hit Rate (HitR), which focuses on the clinical relevance of image registration accuracy. Unlike traditional metrics such as Target Registration Error, which emphasize subresolution differences, HitR considers whether registration algorithms successfully position landmarks within defined confidence zones. This paradigm shift acknowledges the inherent annotation noise in medical images, allowing for more meaningful assessments. To equip HitR with label-noise-awareness, we propose defining these confidence zones based on an Inter-rater Variance analysis. Consequently, hit rate curves are computed for varying landmark zone sizes, enabling performance measurement for a task-specific level of accuracy. Our approach offers a more realistic and meaningful assessment of image registration algorithms, reflecting their suitability for clinical and biomedical applications.

==> body/results/results.tex <==
\section{Experiments}
We demonstrate the application of our proposed metric on a dataset from the BraTS-Reg challenge \citep{baheti2021brain}, evaluating the participating algorithms accordingly.

\input{body/results_data}
\input{body/results_interrater}
\input{body/results_curves}
\input{body/results_runtime}

==> body/results/results_curves.tex <==
\subsection{Hit Rate Curves}
\label{sec:hitrate_curves}

Instead of applying the annotator distances directly (gold standard) for finding suitable radii, we can sample from the distribution according to \Cref{eq:sampling}. 
This results in hit rate curves as shown in \Cref{curves}.

\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/all.png}}
    \caption{Hit rate curves for all competing methods.}
    \label{all}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/first_per_tier.png}}
    \caption{Hit rate curves comparing the best methods per tier.}
    \label{best_per_tier}
\end{subfigure}
\caption{Hit rate curves for (a) all competing methods and (b) best method per tier. Values between fixed thresholds are interpolated.}
\label{curves}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier1.png}}
    \caption{Hit rate curves comparing the methods within tier 1.}
    \label{tier1}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier2.png}}
    \caption{Hit rate curves comparing the methods within tier 2.}
    \label{tier2}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier3.png}}
    \caption{Hit rate curves comparing the methods within tier 3.}
    \label{tier3}
\end{subfigure}
\caption{Hit rate curves for the competing methods within the same tier, respectively.}
\label{tiers_part1}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier4.png}}
    \caption{Hit rate curves comparing the methods within tier 4.}
    \label{tier4}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier5.png}}
    \caption{Hit rate curves comparing the methods within tier 5.}
    \label{tier5}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/tier6.png}}
    \caption{Hit rate curves comparing the methods within tier 6.}
    \label{tier6}
\end{subfigure}
\caption{Hit rate curves for the competing methods within the same tier, respectively.}
\label{tiers_part2}
\end{figure}

==> body/results/results_data.tex <==
\subsection{Data}

\textbf{\emph{Dataset:}} We use data provided by the BraTS-Reg challenge, which validates algorithms for registering brain MR images before and after tumor resection. 
The dataset used for evaluation consists of 50 cases including the baseline (pre-operative) and one follow-up (post-operative) of the same patient. 
For each timepoint, the four MR sequences native T1-weighted (T1), contrast-enhanced T1 (T1-CE), T2-weighted (T2), and T2 Fluid Attenuated Inversion Recovery (FLAIR) are provided, respectively. 
All images are preprocessed to the same anatomical space. Each case comes with expert annotations in the form of corresponding landmarks in the baseline and the follow-up images. 
The number of annotations vary for each case, ranging from 6 to 50 landmarks for one subject. \\

\noindent \textbf{\emph{Algorithms and Evaluation}}: 15 different algorithms, covering a wide range of registration methods -- including iterative as well as Deep Learning-based approaches -- are included in the challenge. 
Evaluation is performed mainly by calculating the TRE between landmarks warped by the participating registration algorithms and the respective reference annotations. 

==> body/results/results_interrater.tex <==
\subsection{Interrater Analysis}
A subset of 16 cases was selected for interrater analysis. The total number of landmarks over the whole subset is 399.
Provided with the landmarks of the first annotator (Rater 1) in the baseline images only, a second annotator (Rater 2) was asked to re-annotate the landmarks in the follow-up images for a subset of 16 cases of the dataset. 
Then, the distances between Rater 1 and Rater 2 are calculated for each landmark following \Cref{eq:TRE} and \Cref{eq:euclidean}. 
The distribution of all rater distances is shown in \Cref{IRR_distribution}. 
For most of the cases, annotators are able to re-annotate landmarks within distances ranging from $0mm$ to around $3mm$. 
Occasionally, raters's annotations differ by up to almost $12mm$. 

\begin{figure}[!htbp]
\centering
\includegraphics[width=\textwidth]{figures/rater_distribution.png}
\caption{Distribution of annotators' distances on a selection of evaluated cases. While for most of the cases, raters re-annotate landmarks within a distance of around $5mm$, few landmarks are re-annotated with distances up to almost $24mm$.} \label{IRR_distribution}
\end{figure}

When annotations from multiple raters are available, we can directly use a respective annotator distance as radius, see \Cref{eq:D}. 
This means that we can compare an algorithm's registration results in form of warped landmarks concretely with an annotator's distance for each landmark specifically. 
We can then compute hit rates using \Cref{eq:metric} for the algorithms and draw a ranking as shown in \Cref{bar_plot}.
This allows us to evaluate an algorithm's registration accuracy by comparison with human expert performance -- representing the gold standard when it comes to assessing the quality of registration results.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\textwidth]{figures/bar_plot.png}
\caption{Hit rate for each algorithm, comparing an algorithms' registered landmarks with the landmark-specific annotator distances for each landmark separately, produced for a subset of the evaluation data. The most successful algorithm achieves a hit rate around $40\%$, while the lowest ranked algorithm shows a hit rate around $10\%$.} \label{bar_plot}
\end{figure}

==> body/results/results_runtime.tex <==
\subsection{Use Cases}

\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{\textwidth}
    {\includegraphics[width=\textwidth]{figures/curve_plt.png}}
    \caption{Hit rate curves comparing three competing algorithms. Dashed lines denote specific thresholds for further evaluation.}
    \label{curve_plt}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    {\includegraphics[width=\textwidth]{figures/runtime1.png}}
    \caption{Runtime vs accuracy for threshold at $0.71mm$ ($median$ annotator distance) for use cases where high accuracy is required.}
    \label{runtime1}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    {\includegraphics[width=\textwidth]{figures/runtime2.png}}
    \caption{Runtime vs accuracy for threshold at $6.03mm$ for use cases where less registration accuracy is required.}
    \label{runtim2}
\end{subfigure}

[TODO reuse this in discussion]
\caption{Comparing registration methods ranked using specific thresholds and their runtime. Depending on the down-stream clinical task, this can help in deciding between computational runtime and registration accuracy. For example, in pre-registering multiple modalities (PET and MRI) for stereotactic biopsy planning, highly accurate registration is mandatory, but the runtime can be neglected. On the other hand, when doing longitudinal registration for evaluation of tumor response, runtime will be prioritized (as this is done on-line while reading the images as they are being acquired), but given the large margin of the RANO criteria (which define how brain tumor response on MRI is to be evaluated) for determining progressive disease ($40\%$ volumetric increase), registration accuracy requirements can be a bit relaxed.}
\label{ranking}
\end{figure}

==> mandatory/conflicts.tex <==
\coi{We declare we don't have conflicts of interest.}

\clearpage

==> mandatory/ethics.tex <==
\ethics{The work follows appropriate ethical standards in conducting research and writing the manuscript, following all applicable laws and regulations regarding treatment of animals or human subjects.}

